Statistical Modeling of FSO Fronthaul Channel for Drone-based Networks

We consider a drone-based communication network, where several drones hover above an area and serve as mobile remote radio heads for a large number of mobile users. We assume that the drones employ free space optical (FSO) links for fronthauling of the users' data to a central unit. The main focus of this paper is to quantify the geometric loss of the FSO channel arising from random fluctuation of the position and orientation of the drones. In particular, we derive upper and lower bounds, corresponding approximate expressions, and a closed-form statistical model for the geometric loss. Simulation results validate our derivations and quantify the FSO channel quality as a function of the drone's instability, i.e., the variation of its position and orientation.

==> Fig/Bounds/Bounds.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{022}[cl][cl]{\matlabtextA Approx. Lower Bound (10a)}%
\psfrag{023}[cl][cl]{\matlabtextA Approx. Upper Bound (10b)}%
\psfrag{024}[cl][cl]{\matlabtextA Prop. Approx. (11)}%
\psfrag{025}[cl][cl]{\matlabtextA Lower Bound (9a)}%
\psfrag{026}[cl][cl]{\matlabtextA Upper Bound (9b)}%
\psfrag{027}[cl][cl]{\matlabtextA Exact (8)}%
\psfrag{028}[cl][cl]{\matlabtextA Non-Practical Regime}%
\psfrag{029}[cl][cl]{\matlabtextA $(f_y,f_z)=(0,0)$ cm}%
\psfrag{030}[cl][cl]{\matlabtextA $(f_y,f_z)=(10,10)$ cm}%
\psfrag{031}[cl][cl]{\matlabtextA $(f_y,f_z)=(20,20)$ cm}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{032}[bc][bc]{\matlabtextB $-10\log_{10}(h_g(\mathbf{r},\boldsymbol{\omega}))$}%
\psfrag{033}[tc][tc]{\matlabtextB $\alpha$ ($\times\pi$)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.05$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.1$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.15$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.25$}%
\psfrag{006}[ct][ct]{\matlabtextC $0.3$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.35$}%
\psfrag{008}[ct][ct]{\matlabtextC $0.4$}%
\psfrag{009}[ct][ct]{\matlabtextC $0.45$}%
\psfrag{010}[ct][ct]{\matlabtextC $0.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextC $10$}%
\psfrag{012}[rc][rc]{\matlabtextC $12$}%
\psfrag{013}[rc][rc]{\matlabtextC $14$}%
\psfrag{014}[rc][rc]{\matlabtextC $16$}%
\psfrag{015}[rc][rc]{\matlabtextC $18$}%
\psfrag{016}[rc][rc]{\matlabtextC $20$}%
\psfrag{017}[rc][rc]{\matlabtextC $22$}%
\psfrag{018}[rc][rc]{\matlabtextC $24$}%
\psfrag{019}[rc][rc]{\matlabtextC $26$}%
\psfrag{020}[rc][rc]{\matlabtextC $28$}%
\psfrag{021}[rc][rc]{\matlabtextC $30$}%
%
%% </ytick>

==> Fig/PDF/PDF.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{033}[cl][cl]{\matlabtextA $\sigma_o=0.2$ mrad}%
\psfrag{034}[cl][cl]{\matlabtextA $\sigma_o=0.1$ mrad}%
\psfrag{035}[cl][cl]{\matlabtextA $\alpha=\pi/4,\beta=5\pi/4$}%
\psfrag{036}[cl][cl]{\matlabtextA $\alpha=0,\beta=\pi/2$}%
\psfrag{037}[cl][cl]{\matlabtextA Prop. Model (15)}%
\psfrag{038}[cl][cl]{\matlabtextA Histogram (8)}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{039}[bc][bc]{\matlabtextB PDF}%
\psfrag{040}[tc][tc]{\matlabtextB $-10\log_{10}(h_g(\mathbf{r},\boldsymbol{\omega}))$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[ct][ct]{\matlabtextC $10$}%
\psfrag{011}[ct][ct]{\matlabtextC $12$}%
\psfrag{012}[ct][ct]{\matlabtextC $14$}%
\psfrag{013}[ct][ct]{\matlabtextC $16$}%
\psfrag{014}[ct][ct]{\matlabtextC $18$}%
\psfrag{015}[ct][ct]{\matlabtextC $20$}%
\psfrag{016}[ct][ct]{\matlabtextC $22$}%
\psfrag{017}[ct][ct]{\matlabtextC $24$}%
\psfrag{018}[ct][ct]{\matlabtextC $26$}%
\psfrag{019}[ct][ct]{\matlabtextC $28$}%
\psfrag{020}[ct][ct]{\matlabtextC $30$}%
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextD $10$}%
\psfrag{001}[ct][ct]{\matlabtextD $12$}%
\psfrag{002}[ct][ct]{\matlabtextD $14$}%
\psfrag{003}[ct][ct]{\matlabtextD $16$}%
\psfrag{004}[ct][ct]{\matlabtextD $18$}%
\psfrag{005}[ct][ct]{\matlabtextD $20$}%
%
%% </xtick>
%
%% <ytick>
%
\providecommand\matlabtextE{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[rc][rc]{\matlabtextE $0$}%
\psfrag{022}[rc][rc]{\matlabtextE $10$}%
\psfrag{023}[rc][rc]{\matlabtextE $20$}%
\psfrag{024}[rc][rc]{\matlabtextE $30$}%
\psfrag{025}[rc][rc]{\matlabtextE $40$}%
\psfrag{026}[rc][rc]{\matlabtextE $50$}%
\psfrag{027}[rc][rc]{\matlabtextE $60$}%
\psfrag{028}[rc][rc]{\matlabtextE $70$}%
\psfrag{029}[rc][rc]{\matlabtextE $80$}%
\psfrag{030}[rc][rc]{\matlabtextE $90$}%
\psfrag{031}[rc][rc]{\matlabtextE $100$}%
\psfrag{032}[rc][rc]{\matlabtextE $110$}%
%
\providecommand\matlabtextF{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{006}[rc][rc]{\matlabtextF $0$}%
\psfrag{007}[rc][rc]{\matlabtextF $10$}%
\psfrag{008}[rc][rc]{\matlabtextF $20$}%
\psfrag{009}[rc][rc]{\matlabtextF $30$}%
%
%% </ytick>

==> Fig/Stat/Stat.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{022}[cl][cl]{\matlabtextA $L=1500$ m}%
\psfrag{023}[cl][cl]{\matlabtextA $L=1000$ m}%
\psfrag{024}[cl][cl]{\matlabtextA $L=800$ m}%
\psfrag{025}[cl][cl]{\matlabtextA Prop. Approx. (11)}%
\psfrag{026}[cl][cl]{\matlabtextA Exact (8)}%
\psfrag{027}[cl][cl]{\matlabtextA $\sigma_p=0$, $\sigma_o=\sigma$ mrad}%
\psfrag{028}[cl][cl]{\matlabtextA $\sigma_p=\sigma$ cm, $\sigma_o=0$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{15}{15}\selectfont\strut}%
\psfrag{029}[bc][bc]{\matlabtextB $-10\log_{10}(\mathsf{E}_{h_g}\{h_g(\mathbf{r},\boldsymbol{\omega})\})$}%
\psfrag{030}[tc][tc]{\matlabtextB $\sigma$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.3$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.4$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{006}[ct][ct]{\matlabtextC $0.6$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.7$}%
\psfrag{008}[ct][ct]{\matlabtextC $0.8$}%
\psfrag{009}[ct][ct]{\matlabtextC $0.9$}%
\psfrag{010}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextC $10$}%
\psfrag{012}[rc][rc]{\matlabtextC $12$}%
\psfrag{013}[rc][rc]{\matlabtextC $14$}%
\psfrag{014}[rc][rc]{\matlabtextC $16$}%
\psfrag{015}[rc][rc]{\matlabtextC $18$}%
\psfrag{016}[rc][rc]{\matlabtextC $20$}%
\psfrag{017}[rc][rc]{\matlabtextC $22$}%
\psfrag{018}[rc][rc]{\matlabtextC $24$}%
\psfrag{019}[rc][rc]{\matlabtextC $26$}%
\psfrag{020}[rc][rc]{\matlabtextC $28$}%
\psfrag{021}[rc][rc]{\matlabtextC $30$}%
%
%% </ytick>
